Bayesian survival analysis with INLA

This tutorial shows how various Bayesian survival models can be fitted using the integrated nested Laplace approximation in a clear, legible, and comprehensible manner using the INLA and INLAjoint R-packages. Such models include accelerated failure time, proportional hazards, mixture cure, competing risks, multi-state, frailty, and joint models of longitudinal and survival data, originally presented in the article "Bayesian survival analysis with BUGS" (Alvares et al., 2021). In addition, we illustrate the implementation of a new joint model for a longitudinal semicontinuous marker, recurrent events, and a terminal event. Our proposal aims to provide the reader with syntax examples for implementing survival models using a fast and accurate approximate Bayesian inferential approach.

==> sections/11-Comparison-MCMC.tex <==
%% ##############################################################
\section{Comparison of the fitted models with MCMC} \label{sec:CMP}

Comparing the model fit between INLA and MCMC is an important step in assessing the computational efficiency and reliability of our approach. In this paper, we have the opportunity to make such a comparison, as a previous work\cite{alvares2021} fitted all the models (with the exception of the last joint model) using the BUGS software. Figure \ref{PostDens} displays the posterior marginals for all the fixed effects in each model in order to assess the agreement between the INLA and MCMC results. As expected, these posterior distributions exhibit a high degree of concordance, indicating that INLA and MCMC yield consistent results. This further underscores the reliability of INLA as an alternative to MCMC, particularly when computational efficiency is of utmost importance. Computation time is an essential consideration in Bayesian modelling, especially when dealing with extensive datasets or complex models. To illustrate the computational efficiency of INLA, we detailed in Table \ref{CompTime} the time required for fitting all the models using both INLA and MCMC. This comparison highlights the substantial time savings achievable with INLA. For example, for the first joint model, INLA delivered results within 9 seconds, whereas MCMC required more than 1 hour to converge to the same posterior distributions (see Figure \ref{PostDens}).

\begin{figure}[p!]
\centering
\includegraphics[scale=0.8]{DensityPlot.pdf}
\caption{Marginal posterior densities for all the fixed effects of the first 7 models fitted with INLA and MCMC.}
\label{PostDens}
\end{figure}

\begin{table}[ht]
\centering
\begin{tabular}{cccccccc}
  \hline
 & AFT & PH & Mixture cure & Competing risk & Multi-state & Frailty & Joint model 1 \\ 
  \hline
INLA & 0.61 & 0.66 & 0.67 & 1.10 & 0.87 & 0.65 & 8.64 \\ 
  MCMC & 64.53 & 89.73 & 179.32 & 444.71 & 337.82 & 73.59 & 4604.40 \\ 
   \hline
\end{tabular}
\caption{Computation time (in seconds) for the first 7 models with INLA and MCMC.}
\label{CompTime}
\end{table}
